Bridging Domain Generalization to Multimodal Domain Generalization via Unified Representations

Domain Generalization (DG) aims to enhance model robustness in unseen or distributionally shifted target domains through training exclusively on source domains. Although existing DG techniques, such as data manipulation, learning strategies, and representation learning, have shown significant progress, they predominantly address single-modal data. With the emergence of numerous multi-modal datasets and increasing demand for multi-modal tasks, a key challenge in Multi-modal Domain Generalization (MMDG) has emerged: enabling models trained on multi-modal sources to generalize to unseen target distributions within the same modality set. Due to the inherent differences between modalities, directly transferring methods from single-modal DG to MMDG typically yields sub-optimal results. These methods often exhibit randomness during generalization due to the invisibility of target domains and fail to consider inter-modal consistency. Applying these methods independently to each modality in the MMDG setting before combining them can lead to divergent generalization directions across different modalities, resulting in degraded generalization capabilities. To address these challenges, we propose a novel approach that leverages Unified Representations to map different paired modalities together, effectively adapting DG methods to MMDG by enabling synchronized multi-modal improvements within the unified space. Additionally, we introduce a supervised disentanglement framework that separates modal-general and modal-specific information, further enhancing the alignment of unified representations. Extensive experiments on benchmark datasets, including EPIC-Kitchens and Human-Animal-Cartoon, demonstrate the effectiveness and superiority of our method in enhancing multi-modal domain generalization.

==> table/epic_osmmdg_ms.tex <==
% \begin{table*}[t!]
% \centering
% \resizebox{1.0\textwidth}{!}{
% \begin{tabular}{l@{~~~~~}cc ccc ccc ccc ccc ccc}
% \hline

%  & &\multicolumn{3}{c}{\textbf{Modality} } &\multicolumn{3}{c}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Avg} }
%  \\
%         &  & Video  & Audio & \multicolumn{1}{c}{Flow} & OS* & UNK & \multicolumn{1}{c}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
% \hline
% % video audio
% {DeepAll} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 38.90 & 50.00 & \multicolumn{1}{c}{43.76}  & 47.69 & 44.64 & \multicolumn{1}{c}{46.12}  & 52.16 & 42.25 & \multicolumn{1}{c}{46.69}  & 46.25 &45.63  & \multicolumn{1}{c}{45.52}  \\

% {Mixup~\cite{zhang2017mixup}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 38.90 & 50.00 & \multicolumn{1}{c}{43.76}  & 47.69 & 44.64 & \multicolumn{1}{c}{46.12}  & 52.16 & 42.25 & \multicolumn{1}{c}{46.69}  & 46.25 &45.63  & \multicolumn{1}{c}{45.52}  \\

% {MM-SADA~\cite{munro2020multi}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 35.41 &  50.00 & \multicolumn{1}{c}{41.46}  & 47.12 & 50.00 & \multicolumn{1}{c}{48.52}  &51.16  & 46.48 & \multicolumn{1}{c}{48.71}  & 44.56 & 48.83 & \multicolumn{1}{c}{46.23}  \\

% {RNA-Net~\cite{planamente2022domain}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} &39.90  & 38.24 & \multicolumn{1}{c}{39.05}  & 43.80 & 53.57 & \multicolumn{1}{c}{48.20}  & 46.29 & 59.15 & \multicolumn{1}{c}{51.94}  & 43.33 & 50.32 & \multicolumn{1}{c}{46.40}  \\

% {MEDIC~\cite{wang2023generalizable}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 38.40 & 55.88 & \multicolumn{1}{c}{45.52}  & 34.44&  69.64& \multicolumn{1}{c}{46.09}   &39.98  &59.15  & \multicolumn{1}{c}{47.71}   &37.61  & 61.56 & \multicolumn{1}{c}{46.44}  \\


% {SimMMDG~\cite{dong2023simmmdg}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} &  34.41& 70.59 & \multicolumn{1}{c}{46.27}  & 46.83 & 51.79 & \multicolumn{1}{c}{49.18}  & 43.19 & 63.38 & \multicolumn{1}{c}{51.37}  & 41.48 & 61.92 & \multicolumn{1}{c}{48.94}  \\


% {MOOSA~\cite{dong2024towards}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 41.90 &82.35& \multicolumn{1}{c}{\textbf{55.54}}  & 45.53 & 64.29 & \multicolumn{1}{c}{\textbf{53.31}}  & 45.52 & 69.01& \multicolumn{1}{c}{\textbf{54.85}}  &44.32  & 71.88 & \multicolumn{1}{c}{\textbf{54.57}} \\

% {DecouMix (ours)} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 41.90 &82.35& \multicolumn{1}{c}{\textbf{55.54}}  & 45.53 & 64.29 & \multicolumn{1}{c}{\textbf{53.31}}  & 45.52 & 69.01& \multicolumn{1}{c}{\textbf{54.85}}  &44.32  & 71.88 & \multicolumn{1}{c}{\textbf{54.57}} \\


% \hline

% % video flow
% {DeepAll} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} &47.88  & 47.06 & \multicolumn{1}{c}{47.47}  & 48.42 & 44.64 & \multicolumn{1}{c}{46.45}  & 50.28 & 36.62 & \multicolumn{1}{c}{42.38}  & 48.86 & 42.77 & \multicolumn{1}{c}{45.43}  \\

% {Mixup~\cite{zhang2017mixup}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 38.90 & 50.00 & \multicolumn{1}{c}{43.76}  & 47.69 & 44.64 & \multicolumn{1}{c}{46.12}  & 52.16 & 42.25 & \multicolumn{1}{c}{46.69}  & 46.25 &45.63  & \multicolumn{1}{c}{45.52}  \\

% {MM-SADA~\cite{munro2020multi}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 44.39 & 47.06 & \multicolumn{1}{c}{45.69}  & 40.20 &48.21  & \multicolumn{1}{c}{43.84}  & 45.96 & 47.89 & \multicolumn{1}{c}{46.90}  & 43.52 & 47.72 & \multicolumn{1}{c}{45.48}  \\

% {RNA-Net~\cite{planamente2022domain}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 48.13 & 50.00 & \multicolumn{1}{c}{49.05}  & 50.72 & 48.21 & \multicolumn{1}{c}{49.44}  & 51.61 & 39.44 & \multicolumn{1}{c}{44.71}  & 50.15 & 45.88 & \multicolumn{1}{c}{47.73}  \\

% {MEDIC~\cite{wang2023generalizable}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 44.14 & 61.76 & \multicolumn{1}{c}{51.49}  & 43.37& 60.71 & \multicolumn{1}{c}{50.60}   & 40.42 & 56.34 & \multicolumn{1}{c}{47.07}   & 42.64 & 59.60 & \multicolumn{1}{c}{49.72}  \\

% {SimMMDG~\cite{dong2023simmmdg}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} &42.14  & 67.65 & \multicolumn{1}{c}{51.93}  & 41.93 & 78.57 & \multicolumn{1}{c}{54.68}  & 41.75 & 64.79 & \multicolumn{1}{c}{50.78}  & 41.94 & 70.34 & \multicolumn{1}{c}{52.46}  \\

% {MOOSA~\cite{dong2024towards}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 45.14 &61.76  & \multicolumn{1}{c}{\textbf{52.16}}  & 50.00 & 62.50 & \multicolumn{1}{c}{\textbf{55.56}}  &  47.84& 54.93 & \multicolumn{1}{c}{\textbf{51.14}}  & 47.66 & 59.73 & \multicolumn{1}{c}{\textbf{52.95}}  \\

% {DecouMix (ours)} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 45.14 &61.76  & \multicolumn{1}{c}{\textbf{52.16}}  & 50.00 & 62.50 & \multicolumn{1}{c}{\textbf{55.56}}  &  47.84& 54.93 & \multicolumn{1}{c}{\textbf{51.14}}  & 47.66 & 59.73 & \multicolumn{1}{c}{\textbf{52.95}}  \\





% \hline


% % audio flow
% {DeepAll} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 40.90 & 44.12 & \multicolumn{1}{c}{42.45}  & 46.25 & 37.50 & \multicolumn{1}{c}{41.42}  & 38.32 & 46.48 & \multicolumn{1}{c}{42.01}  & 41.82 & 42.70 & \multicolumn{1}{c}{41.96}  \\

% {Mixup~\cite{zhang2017mixup}} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 40.90 & 44.12 & \multicolumn{1}{c}{42.45}  & 46.25 & 37.50 & \multicolumn{1}{c}{41.42}  & 38.32 & 46.48 & \multicolumn{1}{c}{42.01}  & 41.82 & 42.70 & \multicolumn{1}{c}{41.96}  \\

% {MM-SADA~\cite{munro2020multi}} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 38.90 & 47.06 & \multicolumn{1}{c}{42.59}  & 45.97 & 42.86 & \multicolumn{1}{c}{44.36}  & 45.52 & 40.85 & \multicolumn{1}{c}{43.05}  & 43.46 & 43.59 & \multicolumn{1}{c}{43.33}  \\

% {RNA-Net~\cite{planamente2022domain}} &  &&  $\checkmark$&  \multicolumn{1}{c}{$\checkmark$} & 37.16 & 52.94 & \multicolumn{1}{c}{43.67}  & 46.69 & 46.43 & \multicolumn{1}{c}{46.56}  &47.51  & 40.85 & \multicolumn{1}{c}{43.93}  & 43.79 &46.74  & \multicolumn{1}{c}{44.72}  \\



% {MEDIC~\cite{wang2023generalizable}} &  & & $\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} &  44.39& 47.06 & \multicolumn{1}{c}{45.69}  & 38.47& 60.71 & \multicolumn{1}{c}{47.10}   &40.53  & 49.30 & \multicolumn{1}{c}{44.49}   & 41.13 & 52.36 & \multicolumn{1}{c}{45.76}  \\

% {SimMMDG~\cite{dong2023SimMMDG}} &  & & $\checkmark$&  \multicolumn{1}{c}{$\checkmark$} & 43.64& 52.94 & \multicolumn{1}{c}{ 47.84}  &  46.54& 67.86 & \multicolumn{1}{c}{55.21}  &36.88  & 60.56 & \multicolumn{1}{c}{45.84}  & 42.35 & 60.45 & \multicolumn{1}{c}{49.63}  \\


% {MOOSA~\cite{dong2024towards}} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 42.64 & 55.88 & \multicolumn{1}{c}{\textbf{48.37}}  &  46.69& 75.00 & \multicolumn{1}{c}{\textbf{57.55}}  &  42.19& 57.75 & \multicolumn{1}{c}{\textbf{48.76}}  & 43.84 & 62.88 & \multicolumn{1}{c}{\textbf{51.56}}  \\

% {DecouMix (ours) } &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 42.64 & 55.88 & \multicolumn{1}{c}{\textbf{48.37}}  &  46.69& 75.00 & \multicolumn{1}{c}{\textbf{57.55}}  &  42.19& 57.75 & \multicolumn{1}{c}{\textbf{48.76}}  & 43.84 & 62.88 & \multicolumn{1}{c}{\textbf{51.56}}  \\



% \hline


% % video audio flow
% {DeepAll} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 39.15 & 50.00 & \multicolumn{1}{c}{43.92}  & 52.45 &  35.71& \multicolumn{1}{c}{42.49}  & 53.82 &  39.44& \multicolumn{1}{c}{45.52}  &48.47  & 41.72 & \multicolumn{1}{c}{43.98}  \\

% {Mixup~\cite{zhang2017mixup}} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 39.15 & 50.00 & \multicolumn{1}{c}{43.92}  & 52.45 &  35.71& \multicolumn{1}{c}{42.49}  & 53.82 &  39.44& \multicolumn{1}{c}{45.52}  &48.47  & 41.72 & \multicolumn{1}{c}{43.98}  \\

% {MM-SADA~\cite{munro2020multi}} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 38.90 & 41.18 & \multicolumn{1}{c}{40.01}  & 45.68 & 51.79 & \multicolumn{1}{c}{48.54}  & 44.41 &54.93  & \multicolumn{1}{c}{49.11}  &43.00  & 49.30 & \multicolumn{1}{c}{45.89}  \\

% {RNA-Net~\cite{planamente2022domain}} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 40.15 & 50.00 & \multicolumn{1}{c}{44.54}  &  48.85&  44.64& \multicolumn{1}{c}{46.65}  & 48.39 & 49.30 & \multicolumn{1}{c}{48.84}  & 45.80 & 47.98 & \multicolumn{1}{c}{46.68}  \\


% {MEDIC~\cite{wang2023generalizable}} &  &$\checkmark$& $\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 43.64 & 64.71 & \multicolumn{1}{c}{52.13}  & 47.84& 64.29 & \multicolumn{1}{c}{54.86}   &  45.29& 59.15 & \multicolumn{1}{c}{51.30}   & 45.59 & 62.72 & \multicolumn{1}{c}{52.76}  \\

% {SimMMDG~\cite{dong2023simmmdg}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{$\checkmark$} & 40.15 & 73.53 & \multicolumn{1}{c}{51.94}  & 45.68 & 78.57 & \multicolumn{1}{c}{57.77}  & 39.09 & 78.87 & \multicolumn{1}{c}{52.27}  & 41.64 & 76.99 & \multicolumn{1}{c}{53.99}  \\




% {MOOSA~\cite{dong2024towards}} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 46.13 &73.52  & \multicolumn{1}{c}{\textbf{56.70}}  &53.03  &  67.86& \multicolumn{1}{c}{\textbf{59.53}}  & 48.84 & 60.56 & \multicolumn{1}{c}{\textbf{54.07}}  & 49.33 & 67.31 & \multicolumn{1}{c}{\textbf{56.77}}  \\

% {DecouMix (ours)} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 46.13 &73.52  & \multicolumn{1}{c}{\textbf{56.70}}  &53.03  &  67.86& \multicolumn{1}{c}{\textbf{59.53}}  & 48.84 & 60.56 & \multicolumn{1}{c}{\textbf{54.07}}  & 49.33 & 67.31 & \multicolumn{1}{c}{\textbf{56.77}}  \\



% \hline
% \end{tabular} 
% }
% % \vspace{0.1cm}
% \caption{Multimodal \textbf{Open-set DG} with different combinations of modalities on EPIC-Kitchens dataset.}
% % \vspace{-0.7cm}
% \label{tab:epic-open} 
% \end{table*}

==> table/hac_osmmdg_ms.tex <==
% \begin{table*}[t!]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l@{~~~~~}cc ccc ccc ccc ccc ccc}
% \hline

%  & &\multicolumn{3}{c}{\textbf{Modality} } &\multicolumn{3}{c}{A, C $\rightarrow$ H } & \multicolumn{3}{c}{H, C $\rightarrow$ A } & \multicolumn{3}{c}{H, A $\rightarrow$ C }  &  \multicolumn{3}{c}{\textit{Avg} }
%  \\
%         &  & Video  & Audio & \multicolumn{1}{c}{Flow} & OS* & UNK & \multicolumn{1}{c}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
% \hline

% {DeepAll} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 62.83 & 60.10 & \multicolumn{1}{c}{61.43}  & 67.40 & 51.13 & \multicolumn{1}{c}{58.15}  & 40.23 & 55.56 & \multicolumn{1}{c}{46.67}  & 56.82 & 55.60 & \multicolumn{1}{c}{55.42}  \\

% {Mixup~\cite{zhang2017mixup}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 62.83 & 60.10 & \multicolumn{1}{c}{61.43}  & 67.40 & 51.13 & \multicolumn{1}{c}{58.15}  & 40.23 & 55.56 & \multicolumn{1}{c}{46.67}  & 56.82 & 55.60 & \multicolumn{1}{c}{55.42}  \\

% {MM-SADA~\cite{munro2020multi}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 62.32 & 77.78 & \multicolumn{1}{c}{69.20}  & 68.95 & 61.65 & \multicolumn{1}{c}{65.10}  & 33.37 & 50.79 & \multicolumn{1}{c}{40.28}  & 54.88 & 63.41 & \multicolumn{1}{c}{58.19}  \\

% {RNA-Net~\cite{planamente2022domain}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} &59.29  & 74.24 & \multicolumn{1}{c}{65.93}  & 72.19 & 58.65 & \multicolumn{1}{c}{64.72}  & 32.33 & 67.46 & \multicolumn{1}{c}{43.71}  & 54.60 & 66.78 & \multicolumn{1}{c}{58.12}  \\


% {MEDIC~\cite{wang2023generalizable}} &  &$\checkmark$&  $\checkmark$&  \multicolumn{1}{c}{} & 51.05 & 80.30 & \multicolumn{1}{c}{62.42}  & 53.69&  75.19& \multicolumn{1}{c}{62.64}   &  35.76&  66.67& \multicolumn{1}{c}{46.55}   & 46.83 & 74.05 & \multicolumn{1}{c}{57.20}  \\

% {SimMMDG~\cite{dong2023simmmdg}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 68.88 & 80.81 & \multicolumn{1}{c}{\textbf{74.37}}   & 59.38 & 75.94 & \multicolumn{1}{c}{66.65}  & 35.97 & 68.25 & \multicolumn{1}{c}{47.11}  & 54.74 & 75.00 & \multicolumn{1}{c}{62.71}  \\

% {MOOSA~\cite{dong2024towards}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 70.40 &  77.78 & \multicolumn{1}{c}{73.90}  & 66.62 & 71.43 & \multicolumn{1}{c}{\textbf{68.94}}  & 36.80 & 76.19 & \multicolumn{1}{c}{\textbf{49.63}}  & 57.94 & 75.13 & \multicolumn{1}{c}{\textbf{64.16}}  \\

% {DecouMix (ours)} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{} & 70.40 &  77.78 & \multicolumn{1}{c}{73.90}  & 66.62 & 71.43 & \multicolumn{1}{c}{\textbf{68.94}}  & 36.80 & 76.19 & \multicolumn{1}{c}{\textbf{49.63}}  & 57.94 & 75.13 & \multicolumn{1}{c}{\textbf{64.16}}  \\



% \hline

% % video flow
% {DeepAll} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 69.05 & 58.59 & \multicolumn{1}{c}{63.39}  & 70.89 & 45.11 & \multicolumn{1}{c}{55.14}  & 40.12 & 64.29 & \multicolumn{1}{c}{49.41}  &  60.02& 56.00 & \multicolumn{1}{c}{55.98}  \\

% {Mixup~\cite{zhang2017mixup}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 69.05 & 58.59 & \multicolumn{1}{c}{63.39}  & 70.89 & 45.11 & \multicolumn{1}{c}{55.14}  & 40.12 & 64.29 & \multicolumn{1}{c}{49.41}  &  60.02& 56.00 & \multicolumn{1}{c}{55.98}  \\

% {MM-SADA~\cite{munro2020multi}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 64.17 & 65.15 & \multicolumn{1}{c}{64.66}  & 65.59 & 62.41 & \multicolumn{1}{c}{63.96}  & 38.36 & 58.73 & \multicolumn{1}{c}{46.41}  & 56.04 & 62.10 & \multicolumn{1}{c}{58.34}  \\

% {RNA-Net~\cite{planamente2022domain}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 74.26 & 53.54 & \multicolumn{1}{c}{62.22}  & 68.08 & 58.65 & \multicolumn{1}{c}{63.44}  & 39.71 & 53.97 & \multicolumn{1}{c}{45.75}  & 60.68 & 55.39 & \multicolumn{1}{c}{57.14}  \\


% {MEDIC~\cite{wang2023generalizable}} &  &$\checkmark$&  &  \multicolumn{1}{c}{$\checkmark$} &58.45  & 76.26 & \multicolumn{1}{c}{66.18}  & 53.17& 69.17 & \multicolumn{1}{c}{60.12}   & 37.01 & 66.67 & \multicolumn{1}{c}{47.59}   & 49.54 & 70.70 & \multicolumn{1}{c}{57.96}  \\


% {SimMMDG~\cite{dong2023simmmdg}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 74.43 & 59.09 & \multicolumn{1}{c}{65.88}  & 61.32 & 72.93 & \multicolumn{1}{c}{66.62}  & 37.42 & 67.46 & \multicolumn{1}{c}{48.14}  & 57.72 & 66.49 & \multicolumn{1}{c}{60.21}  \\

% {MOOSA~\cite{dong2024towards}} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 70.98 & 68.69 & \multicolumn{1}{c}{\textbf{69.82}}  &65.59  & 69.92 & \multicolumn{1}{c}{\textbf{67.69}}  & 45.84 & 63.49 & \multicolumn{1}{c}{\textbf{53.24}}  &  60.80& 67.37 & \multicolumn{1}{c}{\textbf{63.58}}  \\

% {DecouMix (ours)} &  & $\checkmark$& &  \multicolumn{1}{c}{$\checkmark$} & 70.98 & 68.69 & \multicolumn{1}{c}{\textbf{69.82}}  &65.59  & 69.92 & \multicolumn{1}{c}{\textbf{67.69}}  & 45.84 & 63.49 & \multicolumn{1}{c}{\textbf{53.24}}  &  60.80& 67.37 & \multicolumn{1}{c}{\textbf{63.58}}  \\
 


% \hline

% % audio flow
% {DeepAll} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 47.94 & 64.65 & \multicolumn{1}{c}{55.05}  &  60.67& 33.08 & \multicolumn{1}{c}{42.82}  & 33.37 & 50.00 & \multicolumn{1}{c}{40.02}  & 47.33 & 49.24 & \multicolumn{1}{c}{45.96}  \\

% {Mixup~\cite{zhang2017mixup}} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 47.94 & 64.65 & \multicolumn{1}{c}{55.05}  &  60.67& 33.08 & \multicolumn{1}{c}{42.82}  & 33.37 & 50.00 & \multicolumn{1}{c}{40.02}  & 47.33 & 49.24 & \multicolumn{1}{c}{45.96}  \\

% {MM-SADA~\cite{munro2020multi}} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 43.48 & 52.53 & \multicolumn{1}{c}{47.58}  & 44.24 & 53.38 & \multicolumn{1}{c}{48.39}  & 35.34 & 50.00 & \multicolumn{1}{c}{41.41}  &  41.02& 51.97 & \multicolumn{1}{c}{45.79}  \\

% {RNA-Net~\cite{planamente2022domain}} &  &&  $\checkmark$&  \multicolumn{1}{c}{$\checkmark$} & 47.43 & 58.08 & \multicolumn{1}{c}{52.22}  & 56.79 & 42.86 & \multicolumn{1}{c}{48.85}  & 34.82 & 57.14 & \multicolumn{1}{c}{43.27}  &46.35  & 52.69 & \multicolumn{1}{c}{48.11}  \\


% {MEDIC~\cite{wang2023generalizable}} &  && $\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 45.08 &  66.67& \multicolumn{1}{c}{53.79}  & 47.61&  60.90& \multicolumn{1}{c}{53.44}   &  34.62&60.32  & \multicolumn{1}{c}{43.99}   &  42.44& 62.63 & \multicolumn{1}{c}{50.41}  \\

% {SimMMDG~\cite{dong2023simmmdg}} &  & & $\checkmark$&  \multicolumn{1}{c}{$\checkmark$} & 46.93 & 69.70 & \multicolumn{1}{c}{56.09}  & 45.67 & 60.15 & \multicolumn{1}{c}{51.92}  & 36.28 & 66.67 & \multicolumn{1}{c}{\textbf{46.99}} & 42.96 & 65.51 & \multicolumn{1}{c}{51.67}  \\

% {MOOSA~\cite{dong2024towards}} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 45.75 & 76.26 & \multicolumn{1}{c}{\textbf{57.19}}  &51.36 &   59.40 & \multicolumn{1}{c}{\textbf{55.09}}  &36.38 & 64.29 & \multicolumn{1}{c}{46.47}  & 44.50 & 66.65 & \multicolumn{1}{c}{\textbf{52.92}}  \\

% {Decouple (ours)} &  & &$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 45.75 & 76.26 & \multicolumn{1}{c}{\textbf{57.19}}  &51.36 &   59.40 & \multicolumn{1}{c}{\textbf{55.09}}  &36.38 & 64.29 & \multicolumn{1}{c}{46.47}  & 44.50 & 66.65 & \multicolumn{1}{c}{\textbf{52.92}}  \\


% \hline


% % video audio flow
% {DeepAll} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 66.02 &71.72  & \multicolumn{1}{c}{68.75}  & 74.51 & 54.14 & \multicolumn{1}{c}{62.71}  & 44.59 & 55.56 & \multicolumn{1}{c}{49.48}  &  61.71& 60.47 & \multicolumn{1}{c}{60.31}  \\

% {Mixup~\cite{zhang2017mixup}} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 66.02 &71.72  & \multicolumn{1}{c}{68.75}  & 74.51 & 54.14 & \multicolumn{1}{c}{62.71}  & 44.59 & 55.56 & \multicolumn{1}{c}{49.48}  &  61.71& 60.47 & \multicolumn{1}{c}{60.31}  \\

% {MM-SADA~\cite{munro2020multi}} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 60.13 & 72.22 & \multicolumn{1}{c}{65.63}  & 76.46 & 52.63 & \multicolumn{1}{c}{62.35}  &  40.64  & 56.35 & \multicolumn{1}{c}{47.23}  &59.08  & 60.40 & \multicolumn{1}{c}{58.40}  \\

% {RNA-Net~\cite{planamente2022domain}} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 70.31 & 67.68 & \multicolumn{1}{c}{68.97}  & 72.06 & 51.88 & \multicolumn{1}{c}{60.33}  &46.99  &55.56 & \multicolumn{1}{c}{50.91}  & 63.12 & 58.37 & \multicolumn{1}{c}{60.07}  \\


% {MEDIC~\cite{wang2023generalizable}} &  &$\checkmark$& $\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 56.18 & 77.78 & \multicolumn{1}{c}{65.24}  &58.47 & 69.17 & \multicolumn{1}{c}{63.37}   & 42.93 & 61.11 & \multicolumn{1}{c}{50.43}   &  52.53& 69.35 & \multicolumn{1}{c}{59.68}  \\

% {SimMMDG~\cite{dong2023simmmdg}} &  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c}{$\checkmark$} & 62.83 & 77.27 & \multicolumn{1}{c}{69.30}  & 63.78 & 75.19 & \multicolumn{1}{c}{69.01}  & 42.41 & 64.29 & \multicolumn{1}{c}{51.11}  &56.34  & 72.25 & \multicolumn{1}{c}{63.14}  \\

% {MOOSA~\cite{dong2024towards}} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 66.69 & 78.79 & \multicolumn{1}{c}{\textbf{72.24}}  &66.36 & 75.94 & \multicolumn{1}{c}{\textbf{70.83}}  &  45.01& 62.70 & \multicolumn{1}{c}{\textbf{52.40}}  & 59.35& 72.48 & \multicolumn{1}{c}{\textbf{65.16}}  \\

% {DecouMix (ours)} &  & $\checkmark$&$\checkmark$ &  \multicolumn{1}{c}{$\checkmark$} & 66.69 & 78.79 & \multicolumn{1}{c}{\textbf{72.24}}  &66.36 & 75.94 & \multicolumn{1}{c}{\textbf{70.83}}  &  45.01& 62.70 & \multicolumn{1}{c}{\textbf{52.40}}  & 59.35& 72.48 & \multicolumn{1}{c}{\textbf{65.16}}  \\


% \hline
% \end{tabular} 
% }
% \vspace{0.1cm}
% \caption{Multimodal \textbf{Open-set DG} with different combinations of modalities on HAC dataset.}
% \label{tab:hac-open} 
% \end{table*}

==> table/modal_compete_full.tex <==
\begin{table}[]
    \centering
    \setlength{\tabcolsep}{10pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lcccc}
\toprule
& \multicolumn{4}{c}{\textbf{EPIC-Kitchens}}  \\
\cmidrule(lr){2-5} \textbf{Method} & Video & Audio & Flow & V-A-F\\
\midrule
Base (V) &  58.73 & - & - & -\\
Base (A) &  - & 40.04 & - & -\\
Base (F) &  - & - & 57.61 & -\\
Base (VAF) &  57.13 & 37.96 & 56.65 & 61.20\\
\midrule
JiGen (V) & 61.60 & - & - & -\\
JiGen (A) &  - &  42.06 & - & -\\
JiGen (F) &  - & - &  59.85 & -\\
JiGen (VAF) &  59.23 & 39.58 & 57.18 & 62.81\\
\midrule
Mixup (V) &  \underline{61.92} & - & - & -\\
Mixup (A) &  - & 42.74 & - & -\\
Mixup (F) &  - & - & 60.16 & -\\
Mixup (VAF) &  58.98 & 40.67 & 58.25 & 63.42\\
\midrule
UR-JiGen (VAF) &  61.72 & \underline{43.41} & \underline{60.67} & \underline{67.04}\\
UR-Mixup (VAF) &  \textbf{62.45} & \textbf{43.79} & \textbf{61.37} & \textbf{67.79}\\
\bottomrule
    \end{tabular}}
    \caption{MMDG analysis on EPIC-Kitchens using video, audio, and flow data, with results reported in accuracy (\%). 'Base' denotes vanilla multi-modal joint training without domain generalization. Parentheses indicate training modalities: V (Video), A (Audio), and F (Flow). 'Video,' 'Audio,' 'Flow,' and 'V-A-F' represent uni-modal and multi-modal testing. Results are averaged by using each domain as target.
}
    \label{tab:modal_compete}
\vspace{-5mm}
\end{table}

% \begin{table}[h]
% \centering
% \resizebox{0.6\linewidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{4}{c}{\textbf{EPIC-Kitchens}} 
% \cmidrule(lr){2-5} \\
% \textbf{Method} & Video & Audio & Flow & V-A-F\\
% \midrule
% Base(V) &  58.73 & - & - & -\\
% Base(A) &  - & 40.04 & - & -\\
% Base(F) &  - & - & 52.61 & -\\
% Mixup(V) & 56.30 & - & - & -\\
% Mixup(A) &  - &  40.35 & - & -\\
% Mixup(F) &  - & - &  58.85 & -\\
% JiGen(V) &  58.73 & - & - & -\\
% JiGen(A) &  - & 40.04 & - & -\\
% JiGen(F) &  - & - & 52.61 & -\\
% \midrule
% Base(VAF) &  - & - & - & 61.20\\
% Mixup(VAF) &  - & - & - & 61.20\\
% JiGen(VAF) &  - & - & - & 61.20\\
% \bottomrule
% \end{tabular}
% }
% \caption{Modal_compete}
% \label{tab:epic-dg2}
% \end{table}

==> table/single_modal_DG.tex <==
% \begin{table}[h!]
% \centering
% \begin{adjustbox}{width=0.98\linewidth}
% \begin{tabular}{lcccc}
% \toprule
% %Method & \makecell[c]{D2, D3 \\ $\rightarrow$ D1} & \makecell[c]{D1, D3 \\ $\rightarrow$ D2} & \makecell[c]{D1, D2 \\ $\rightarrow$ D3}  & \textit{Mean}\\
% \textbf{Method} &D2, D3 $\rightarrow$ D1 & D1, D3 $\rightarrow$ D2 & D1, D2 $\rightarrow$ D3  & \textit{Mean}\\
%  \noalign{\smallskip} \hline \noalign{\smallskip} 
% Mixup (V) & 49.20 & 59.73 &59.96 &56.30\\ 
% Mixup (A) & 35.17 &  40.80&45.07 & 40.35\\ 
% Mixup (F) &56.32  & 65.60 & 54.62&58.85\\  
% Mixup (V+A+F) &56.32  & 65.60 & 54.62&58.85\\ 
% JiGen (V) & 49.20 & 59.73 &59.96 &56.30\\ 
% JiGen (A) & 35.17 &  40.80&45.07 & 40.35\\ 
% JiGen (F) &56.32  & 65.60 & 54.62&58.85\\  
% JiGen (V+A+F) &56.32  & 65.60 & 54.62&58.85\\
% \bottomrule
% \end{tabular}
% \end{adjustbox}

% %\vspace{+0.05cm}
% %\caption{Comparison with single-modal DG methods on EPIC-Kitchens dataset. V: video, A: audio, F: optical flow.}
% %\vspace{-1cm}

% \label{tab:single-re}
% \end{table}




==> table/sup_af_compete.tex <==
\begin{table*}[]
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{\textbf{EPIC-Kitchens}} & \multicolumn{3}{c}{\textbf{HAC}}  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \textbf{Method} & Audio & Flow & Audio-Flow  & Audio & Flow & Audio-Flow\\
\midrule
Base (A) &  40.04 & - & - & 32.81 & - & -& 32.81 & - & -\\
Base (F) &  - & 58.30 & - & - & 53.20 & -\\
Base (AF) & 39.42 & 54.86 & 53.14 &30.28 & 50.39 & 49.64\\
\midrule
JiGen (A) & 42.72 & - & - & 35.26 & - & -\\
JiGen (F) & - & \underline{60.77} & - & - & 54.36 & -\\
JiGen (AF) &40.26 & 56.38 & 58.93  & 31.14 & 51.50 & 54.57\\
\midrule
Mixup (A) &\underline{43.74} & - & - & \underline{35.83} & - & -\\
Mixup (F) &- & \textbf{60.89} & - & - & \underline{54.84} & -\\
Mixup (AF) &40.38 & 57.08 & 58.32 & 32.43 & 51.76 & 55.09\\
\midrule
UR-JiGen (AF) & 43.52 & \textbf{60.89} & \textbf{63.32}  & 35.69 & 53.97 & \underline{58.56}\\
UR-Mixup (AF) & \textbf{44.24} & 60.24 & \underline{62.63} & \textbf{36.27} & \textbf{55.08} & \textbf{58.84}\\
\bottomrule
    \end{tabular}}
    \caption{MMDG analysis on EPIC-Kitchens and HAC using audio, flow data. 'Base' denotes vanilla multi-modal joint training without domain generalization. Parentheses indicate training modalities: A (Audio) and F (Flow). 'Audio', 'Flow' and 'Audio-Flow' represent uni-modal and multi-modal testing. Results are averaged by using each domain as target.
}
    \label{tab:sup_va_compete}
\end{table*}

% \begin{table}[h]
% \centering
% \resizebox{0.6\linewidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{4}{c}{\textbf{EPIC-Kitchens}} 
% \cmidrule(lr){2-5} \\
% \textbf{Method} & Video & Audio & Flow & V-A-F\\
% \midrule
% Base(V) &  58.73 & - & - & -\\
% Base(A) &  - & 40.04 & - & -\\
% Base(F) &  - & - & 52.61 & -\\
% Mixup(V) & 56.30 & - & - & -\\
% Mixup(A) &  - &  40.35 & - & -\\
% Mixup(F) &  - & - &  58.85 & -\\
% JiGen(V) &  58.73 & - & - & -\\
% JiGen(A) &  - & 40.04 & - & -\\
% JiGen(F) &  - & - & 52.61 & -\\
% \midrule
% Base(VAF) &  - & - & - & 61.20\\
% Mixup(VAF) &  - & - & - & 61.20\\
% JiGen(VAF) &  - & - & - & 61.20\\
% \bottomrule
% \end{tabular}
% }
% \caption{Modal_compete}
% \label{tab:epic-dg2}
% \end{table}

==> table/sup_epic_hac_UR_add.tex <==
% \begin{table*}[t!]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{cccccccccccc}
% \toprule
% \multicolumn{3}{c}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{EPIC-Kitchens dataset}}& \multicolumn{4}{c}{\textbf{HAC dataset}}\\
% \cmidrule(lr){1-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11} %:)
% Mixup & JiGen & IBN & D2, D3 $\rightarrow$ D1 & D1, D3 $\rightarrow$ D2 & D1, D2 $\rightarrow$ D3  & \textit{Avg} & A, C $\rightarrow$ H & H, C $\rightarrow$ A & H, A $\rightarrow$ C  & \textit{Avg}\\

% \midrule
% \rowcolor{gray!30} 
% $\checkmark$& -& - & 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% \rowcolor{gray!30} 
% -&$\checkmark$& -&  55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% \rowcolor{gray!30} 
% -& -&$\checkmark$& 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% \rowcolor{gray!30} 
% $\checkmark$& $\checkmark$& - & 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% \rowcolor{gray!30} 
% $\checkmark$& -& $\checkmark$ & 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% \rowcolor{gray!30} 
% $\checkmark$& $\checkmark$& $\checkmark$ & 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\

% $\checkmark$& -& - & 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% -&$\checkmark$& -&  55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% -& -&$\checkmark$& 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% $\checkmark$& $\checkmark$& - & 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% $\checkmark$& -& $\checkmark$ & 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\
% $\checkmark$& $\checkmark$& $\checkmark$ & 55.63 & 59.20 & 58.01 & 57.61& 69.07&  71.30 &51.47 & 63.95  \\

% \bottomrule
% \end{tabular}

% \end{threeparttable}
% }
% %\vspace{-0.5em}
% \caption{Multi-modal \textbf{multi-source} DG with different modalities on EPIC-Kitchens and HAC datasets.}
% %\vspace{-0.8em}
% \label{tab:epic-dg2}
% \end{table*}

==> table/sup_epic_singlesource.tex <==

\begin{table*}[t!]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lccccccccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Modality}} & \multicolumn{2}{c}{\textbf{Source: D1}}& \multicolumn{2}{c}{\textbf{Source: D2}}& \multicolumn{2}{c}{\textbf{Source: D3}}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
\textbf{Method} & Video & Audio & Flow & D1$\rightarrow$ D2 & D1$\rightarrow$ D3 & D2 $\rightarrow$ D1 & D2 $\rightarrow$ D3& D3$\rightarrow$ D1& D3$\rightarrow$ D2  & \textit{Mean}\\
%\midrule

%RSC (flow-only) & & &$\checkmark$ & 55.17  & 63.33  &     59.65 &  59.38  \\
%Mixup (flow-only) & & &$\checkmark$ & 56.32   &  61.07 &   54.62   & 57.34   \\

\midrule
DeepAll & $\checkmark$& &$\checkmark$ &53.07  & 47.74 &49.66 & 56.98&\textbf{52.18}  & 55.73&52.56  \\
MM-SADA~\cite{Munro_2020_CVPR} & $\checkmark$& &$\checkmark$ &  49.20& 48.87 & 51.26&59.03 &44.60 & 56.40& 51.56 \\
RNA-Net~\cite{Planamente_2022_WACV} & $\checkmark$& & $\checkmark$& 53.20& 49.79 & 52.18&58.11 & 47.13&55.47 & 52.65 \\
SimMMDG~\cite{dong2023simmmdg}  & $\checkmark$& & $\checkmark$& \textbf{56.80} & \textbf{54.11} & \textbf{53.10} & \textbf{59.86}  & 50.57& \textbf{64.27} & \textbf{56.45}\\
CMRF~\cite{CMRF}  & $\checkmark$& & $\checkmark$& \textbf{56.80} & \textbf{54.11} & \textbf{53.10} & \textbf{59.86}  & 50.57& \textbf{64.27} & \textbf{56.45}\\
\rowcolor{gray!30} 
Mixup~\cite{zhang2017mixup}  & $\checkmark$& & $\checkmark$& \textbf{56.80} & \textbf{54.11} & \textbf{53.10} & \textbf{59.86}  & 50.57& \textbf{64.27} & \textbf{56.45}\\
\rowcolor{gray!30} 
JiGen~\cite{zhang2017mixup}  & $\checkmark$& & $\checkmark$& \textbf{56.80} & \textbf{54.11} & \textbf{53.10} & \textbf{59.86}  & 50.57& \textbf{64.27} & \textbf{56.45}\\
\rowcolor{gray!30} 
IBN~\cite{zhang2017mixup}  & $\checkmark$& & $\checkmark$& \textbf{56.80} & \textbf{54.11} & \textbf{53.10} & \textbf{59.86}  & 50.57& \textbf{64.27} & \textbf{56.45}\\
UR-Mixup~\cite{zhang2017mixup}  & $\checkmark$& & $\checkmark$& \textbf{56.80} & \textbf{54.11} & \textbf{53.10} & \textbf{59.86}  & 50.57& \textbf{64.27} & \textbf{56.45}\\
\rowcolor{gray!30} 
UR-JiGen~\cite{zhang2017mixup}  & $\checkmark$& & $\checkmark$& \textbf{56.80} & \textbf{54.11} & \textbf{53.10} & \textbf{59.86}  & 50.57& \textbf{64.27} & \textbf{56.45}\\
\rowcolor{gray!30} 
UR-IBN~\cite{zhang2017mixup}  & $\checkmark$& & $\checkmark$& \textbf{56.80} & \textbf{54.11} & \textbf{53.10} & \textbf{59.86}  & 50.57& \textbf{64.27} & \textbf{56.45}\\

\midrule
DeepAll & & $\checkmark$&$\checkmark$ & 41.60 &  47.43&41.61 &51.75 &45.98 & 56.13& 47.42 \\
MM-SADA~\cite{Munro_2020_CVPR} & &$\checkmark$ &$\checkmark$ &42.53 & 47.64 &42.76 & 50.92& 42.07& 51.87& 46.30 \\
RNA-Net~\cite{Planamente_2022_WACV} & & $\checkmark$&$\checkmark$ & 46.40 & 49.38 &42.76 & 54.62&43.45 & 52.13& 48.12 \\
SimMMDG~\cite{dong2023simmmdg}  & & $\checkmark$&$\checkmark$ & \textbf{50.00} & \textbf{49.49} & \textbf{45.98} & \textbf{56.26}  & \textbf{51.95} & \textbf{63.87} & \textbf{52.93}\\
CMRF~\cite{CMRF}  & & $\checkmark$&$\checkmark$ & \textbf{50.00} & \textbf{49.49} & \textbf{45.98} & \textbf{56.26}  & \textbf{51.95} & \textbf{63.87} & \textbf{52.93}\\
\rowcolor{gray!30} 
Mixup~\cite{CMRF}  & & $\checkmark$&$\checkmark$ & \textbf{50.00} & \textbf{49.49} & \textbf{45.98} & \textbf{56.26}  & \textbf{51.95} & \textbf{63.87} & \textbf{52.93}\\
\rowcolor{gray!30} 
JiGen~\cite{CMRF}  & & $\checkmark$&$\checkmark$ & \textbf{50.00} & \textbf{49.49} & \textbf{45.98} & \textbf{56.26}  & \textbf{51.95} & \textbf{63.87} & \textbf{52.93}\\
\rowcolor{gray!30} 
IBN~\cite{CMRF}  & & $\checkmark$&$\checkmark$ & \textbf{50.00} & \textbf{49.49} & \textbf{45.98} & \textbf{56.26}  & \textbf{51.95} & \textbf{63.87} & \textbf{52.93}\\
UR-Mixup~\cite{CMRF}  & & $\checkmark$&$\checkmark$ & \textbf{50.00} & \textbf{49.49} & \textbf{45.98} & \textbf{56.26}  & \textbf{51.95} & \textbf{63.87} & \textbf{52.93}\\
\rowcolor{gray!30} 
UR-JiGen~\cite{CMRF}  & & $\checkmark$&$\checkmark$ & \textbf{50.00} & \textbf{49.49} & \textbf{45.98} & \textbf{56.26}  & \textbf{51.95} & \textbf{63.87} & \textbf{52.93}\\
\rowcolor{gray!30} 
UR-IBN~\cite{CMRF}  & & $\checkmark$&$\checkmark$ & \textbf{50.00} & \textbf{49.49} & \textbf{45.98} & \textbf{56.26}  & \textbf{51.95} & \textbf{63.87} & \textbf{52.93}\\

\midrule
DeepAll & $\checkmark$& $\checkmark$& $\checkmark$ & 51.60 & 53.39 &44.60 & \textbf{60.16} &45.74 &53.47 &  51.49\\
MM-SADA~\cite{Munro_2020_CVPR} & $\checkmark$&$\checkmark$ &$\checkmark$ &49.43  & 48.53 & 38.16&48.46 &44.14 & 51.07& 46.63 \\
RNA-Net~\cite{Planamente_2022_WACV} & $\checkmark$& $\checkmark$& $\checkmark$ &  51.20&  53.90&46.67 & 58.73&49.43 & 57.47& 52.90 \\
SimMMDG~\cite{dong2023simmmdg}  & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{55.33} & \textbf{54.83} & \textbf{50.80} & 59.45  & \textbf{53.33} & \textbf{64.40} & \textbf{56.36}\\
CMRF~\cite{CMRF}  & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{55.33} & \textbf{54.83} & \textbf{50.80} & 59.45  & \textbf{53.33} & \textbf{64.40} & \textbf{56.36}\\
\rowcolor{gray!30} 
Mixup~\cite{CMRF}  & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{55.33} & \textbf{54.83} & \textbf{50.80} & 59.45  & \textbf{53.33} & \textbf{64.40} & \textbf{56.36}\\
\rowcolor{gray!30} 
JiGen~\cite{CMRF}  & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{55.33} & \textbf{54.83} & \textbf{50.80} & 59.45  & \textbf{53.33} & \textbf{64.40} & \textbf{56.36}\\
\rowcolor{gray!30} 
IBN~\cite{CMRF}  & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{55.33} & \textbf{54.83} & \textbf{50.80} & 59.45  & \textbf{53.33} & \textbf{64.40} & \textbf{56.36}\\
UR-Mixup~\cite{CMRF}  & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{55.33} & \textbf{54.83} & \textbf{50.80} & 59.45  & \textbf{53.33} & \textbf{64.40} & \textbf{56.36}\\
\rowcolor{gray!30} 
UR-JiGen~\cite{CMRF}  & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{55.33} & \textbf{54.83} & \textbf{50.80} & 59.45  & \textbf{53.33} & \textbf{64.40} & \textbf{56.36}\\
\rowcolor{gray!30} 
UR-IBN~\cite{CMRF}  & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{55.33} & \textbf{54.83} & \textbf{50.80} & 59.45  & \textbf{53.33} & \textbf{64.40} & \textbf{56.36}\\


\bottomrule
\end{tabular}

\end{threeparttable}
}
%\vspace{-0.5em}
\caption{Multi-modal \textbf{single-source} DG  with different modalities on EPIC-Kitchens dataset.}
%\vspace{-0.8em}
\label{tab:epic-ssdg-appen}
\end{table*}

==> table/sup_hac_singlesource.tex <==

\begin{table*}[t!]
\centering
\resizebox{0.8\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lccccccccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Modality}} & \multicolumn{2}{c}{\textbf{Source: H}}& \multicolumn{2}{c}{\textbf{Source: A}}& \multicolumn{2}{c}{\textbf{Source: C}}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
\textbf{Method} & Video & Audio & Flow & H$\rightarrow$ A & H$\rightarrow$ C & A $\rightarrow$ H & A $\rightarrow$ C& C$\rightarrow$ H& C$\rightarrow$ A  & \textit{Mean}\\

\midrule
DeepAll & $\checkmark$& &$\checkmark$ &59.82  &41.08  &73.25 & 35.02& 60.71&64.46 & 55.72 \\
MM-SADA~\cite{Munro_2020_CVPR} & $\checkmark$& &$\checkmark$ & \textbf{66.23} & \textbf{46.23} &69.65 & 42.46&59.77 &57.62 &56.99  \\
RNA-Net~\cite{Planamente_2022_WACV} & $\checkmark$& & $\checkmark$& 58.61& 37.87 & 73.90&48.16 &60.35 &59.38 & 56.38 \\
SimMMDG~\cite{dong2023simmmdg} & $\checkmark$& & $\checkmark$& 63.13 & 44.58 & \textbf{74.62} & \textbf{51.38}  & \textbf{70.15} & \textbf{61.59} & \textbf{60.91}\\
CMRF~\cite{CMRF} & $\checkmark$& & $\checkmark$& 63.13 & 44.58 & \textbf{74.62} & \textbf{51.38}  & \textbf{70.15} & \textbf{61.59} & \textbf{60.91}\\
\rowcolor{gray!30} 
Mixup~\cite{CMRF} & $\checkmark$& & $\checkmark$& 63.13 & 44.58 & \textbf{74.62} & \textbf{51.38}  & \textbf{70.15} & \textbf{61.59} & \textbf{60.91}\\
\rowcolor{gray!30} 
JiGen~\cite{CMRF} & $\checkmark$& & $\checkmark$& 63.13 & 44.58 & \textbf{74.62} & \textbf{51.38}  & \textbf{70.15} & \textbf{61.59} & \textbf{60.91}\\
\rowcolor{gray!30} 
IBN~\cite{CMRF} & $\checkmark$& & $\checkmark$& 63.13 & 44.58 & \textbf{74.62} & \textbf{51.38}  & \textbf{70.15} & \textbf{61.59} & \textbf{60.91}\\
UR-Mixup~\cite{CMRF} & $\checkmark$& & $\checkmark$& 63.13 & 44.58 & \textbf{74.62} & \textbf{51.38}  & \textbf{70.15} & \textbf{61.59} & \textbf{60.91}\\
UR-JiGen~\cite{CMRF} & $\checkmark$& & $\checkmark$& 63.13 & 44.58 & \textbf{74.62} & \textbf{51.38}  & \textbf{70.15} & \textbf{61.59} & \textbf{60.91}\\
UR-IBN~\cite{CMRF} & $\checkmark$& & $\checkmark$& 63.13 & 44.58 & \textbf{74.62} & \textbf{51.38}  & \textbf{70.15} & \textbf{61.59} & \textbf{60.91}\\

\midrule
DeepAll & & $\checkmark$&$\checkmark$ & 59.93 & 35.29 & 50.90&35.20 & 32.73& 39.85& 42.32 \\
MM-SADA~\cite{Munro_2020_CVPR} & &$\checkmark$ &$\checkmark$ &55.08 & 32.90 & 52.85&34.10 & 29.70& 44.48&  41.52\\
RNA-Net~\cite{Planamente_2022_WACV} & & $\checkmark$&$\checkmark$ & 56.51 & 30.24 &53.50 & 33.46&36.91 &40.40 & 41.84 \\
SimMMDG~\cite{dong2023simmmdg} & & $\checkmark$&$\checkmark$ & \textbf{62.25} & \textbf{36.40} & \textbf{56.60} & \textbf{38.79}  & \textbf{38.72} & \textbf{48.12} & \textbf{46.81}\\
CMRF~\cite{CMRF} & & $\checkmark$&$\checkmark$ & \textbf{62.25} & \textbf{36.40} & \textbf{56.60} & \textbf{38.79}  & \textbf{38.72} & \textbf{48.12} & \textbf{46.81}\\
\rowcolor{gray!30} 
Mixup~\cite{CMRF} & & $\checkmark$&$\checkmark$ & \textbf{62.25} & \textbf{36.40} & \textbf{56.60} & \textbf{38.79}  & \textbf{38.72} & \textbf{48.12} & \textbf{46.81}\\
\rowcolor{gray!30} 
JiGen~\cite{CMRF} & & $\checkmark$&$\checkmark$ & \textbf{62.25} & \textbf{36.40} & \textbf{56.60} & \textbf{38.79}  & \textbf{38.72} & \textbf{48.12} & \textbf{46.81}\\
\rowcolor{gray!30} 
IBN~\cite{CMRF} & & $\checkmark$&$\checkmark$ & \textbf{62.25} & \textbf{36.40} & \textbf{56.60} & \textbf{38.79}  & \textbf{38.72} & \textbf{48.12} & \textbf{46.81}\\
UR-Mixup~\cite{CMRF} & & $\checkmark$&$\checkmark$ & \textbf{62.25} & \textbf{36.40} & \textbf{56.60} & \textbf{38.79}  & \textbf{38.72} & \textbf{48.12} & \textbf{46.81}\\
UR-JiGen~\cite{CMRF} & & $\checkmark$&$\checkmark$ & \textbf{62.25} & \textbf{36.40} & \textbf{56.60} & \textbf{38.79}  & \textbf{38.72} & \textbf{48.12} & \textbf{46.81}\\
UR-IBN~\cite{CMRF} & & $\checkmark$&$\checkmark$ & \textbf{62.25} & \textbf{36.40} & \textbf{56.60} & \textbf{38.79}  & \textbf{38.72} & \textbf{48.12} & \textbf{46.81}\\

\midrule
DeepAll & $\checkmark$& $\checkmark$& $\checkmark$ & 62.58 & 42.56 &67.34 &46.05 &53.86 &59.49 & 55.31 \\
MM-SADA~\cite{Munro_2020_CVPR} & $\checkmark$&$\checkmark$ &$\checkmark$ &  62.25& 44.67 &60.78 & 43.11&41.82 &44.81 & 49.57 \\
RNA-Net~\cite{Planamente_2022_WACV} & $\checkmark$& $\checkmark$& $\checkmark$ & 66.89 & 45.40 &66.62 &46.88 &53.64 & 61.37& 56.80 \\
SimMMDG~\cite{dong2023simmmdg} & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{68.76} & \textbf{47.98} & \textbf{70.94} & \textbf{49.26}  & \textbf{65.18} & \textbf{62.69} & \textbf{60.80}\\
CMRF~\cite{CMRF} & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{68.76} & \textbf{47.98} & \textbf{70.94} & \textbf{49.26}  & \textbf{65.18} & \textbf{62.69} & \textbf{60.80}\\
\rowcolor{gray!30} 
Mixup~\cite{CMRF} & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{68.76} & \textbf{47.98} & \textbf{70.94} & \textbf{49.26}  & \textbf{65.18} & \textbf{62.69} & \textbf{60.80}\\
\rowcolor{gray!30} 
JiGen~\cite{CMRF} & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{68.76} & \textbf{47.98} & \textbf{70.94} & \textbf{49.26}  & \textbf{65.18} & \textbf{62.69} & \textbf{60.80}\\
\rowcolor{gray!30} 
IBN~\cite{CMRF} & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{68.76} & \textbf{47.98} & \textbf{70.94} & \textbf{49.26}  & \textbf{65.18} & \textbf{62.69} & \textbf{60.80}\\
UR-Mixup~\cite{CMRF} & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{68.76} & \textbf{47.98} & \textbf{70.94} & \textbf{49.26}  & \textbf{65.18} & \textbf{62.69} & \textbf{60.80}\\
UR-JiGen~\cite{CMRF} & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{68.76} & \textbf{47.98} & \textbf{70.94} & \textbf{49.26}  & \textbf{65.18} & \textbf{62.69} & \textbf{60.80}\\
UR-IBN~\cite{CMRF} & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{68.76} & \textbf{47.98} & \textbf{70.94} & \textbf{49.26}  & \textbf{65.18} & \textbf{62.69} & \textbf{60.80}\\
\bottomrule
\end{tabular}

\end{threeparttable}
}
%\vspace{-0.5em}
\caption{Multi-modal \textbf{single-source} DG  with different modalities on HAC dataset.}
%\vspace{-0.8em}
\label{tab:hac-ssdg-appen}
\end{table*}

==> table/sup_va_compete.tex <==
\begin{table*}[]
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{\textbf{EPIC-Kitchens}} & \multicolumn{3}{c}{\textbf{HAC}}  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \textbf{Method} & Video & Audio & Video-Audio  & Video & Audio & Video-Audio\\
\midrule
Base (V) &  58.73 & - & - & 68.07 & - & -\\
Base (A) &  - & 40.04 & - & - & 32.81 & -\\
Base (VA) &  56.65& 38.62& 59.63& 67.60& 31.24& 63.11\\
\midrule
JiGen (V) & 61.60 & - & - & 70.41 & - & -\\
JiGen (A) &  - &  42.72 & - & - & 35.26 & -\\
JiGen (VA) &  58.98 & 40.67 & 61.08 & 63.42& - & 65.80\\
\midrule
Mixup (V) &  61.92 & - & - &\underline{71.12}& - & -\\
Mixup (A) &  - & \underline{43.74} & - & -& \underline{35.83} & -\\
Mixup (VA) &58.52 & 39.31 & 61.18 & 68.22 & 31.64 & 66.41\\
\midrule
UR-JiGen (VA) &  \underline{62.02} & 43.41 & \underline{63.63} & 70.79& 35.14 & \underline{71.40}\\
UR-Mixup (VA) &  \textbf{62.45} & \textbf{43.79} & \textbf{64.77} & \textbf{71.64} & \textbf{36.21} & \textbf{72.36}\\
\bottomrule
    \end{tabular}}
    \caption{MMDG analysis on EPIC-Kitchens and HAC using video, audio data. 'Base' denotes vanilla multi-modal joint training without domain generalization. Parentheses indicate training modalities: V (Video), A (Audio). 'Video', 'Audio' and 'Video-Audio' represent uni-modal and multi-modal testing. Results are averaged by using each domain as target.
}
    \label{tab:sup_va_compete}
\end{table*}

% \begin{table}[h]
% \centering
% \resizebox{0.6\linewidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{4}{c}{\textbf{EPIC-Kitchens}} 
% \cmidrule(lr){2-5} \\
% \textbf{Method} & Video & Audio & Flow & V-A-F\\
% \midrule
% Base(V) &  58.73 & - & - & -\\
% Base(A) &  - & 40.04 & - & -\\
% Base(F) &  - & - & 52.61 & -\\
% Mixup(V) & 56.30 & - & - & -\\
% Mixup(A) &  - &  40.35 & - & -\\
% Mixup(F) &  - & - &  58.85 & -\\
% JiGen(V) &  58.73 & - & - & -\\
% JiGen(A) &  - & 40.04 & - & -\\
% JiGen(F) &  - & - & 52.61 & -\\
% \midrule
% Base(VAF) &  - & - & - & 61.20\\
% Mixup(VAF) &  - & - & - & 61.20\\
% JiGen(VAF) &  - & - & - & 61.20\\
% \bottomrule
% \end{tabular}
% }
% \caption{Modal_compete}
% \label{tab:epic-dg2}
% \end{table}

==> table/sup_vf_compete.tex <==
\begin{table*}[]
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{\textbf{EPIC-Kitchens}} & \multicolumn{3}{c}{\textbf{HAC}}  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \textbf{Method} & Video & Flow & Video-Flow  & Video & Flow & Video-Flow\\
\midrule
Base (V) &  58.73 & - & - & 68.07 & - & -\\
Base (F) &  - & 58.30 & - & - & 53.20 & -\\
Base (VF) & 55.28 & 55.78 & 60.89 & 64.29 & 48.64 & 64.75\\
\midrule
JiGen (V) & 61.60 & - & - & 70.41 & - & -\\
JiGen (F) & - & 60.77 & - & - & 54.36 & -\\
JiGen (VF) &57.14 & 56.64 & 61.79 & 66.28 & 51.87 & 68.12\\
\midrule
Mixup (V) &\underline{61.92} & - & - & 71.12 & - & -\\
Mixup (F) &- & 60.89 & - & - & \textbf{54.84} & -\\
Mixup (VF) &57.86 & 57.24 & 62.08 & 66.71 & 52.48 & 68.93\\
\midrule
UR-JiGen (VF) & 61.26 & \underline{61.08} & \underline{64.15} & \underline{69.89} & \underline{54.74} & \underline{72.31}\\
UR-Mixup (VF) &\textbf{62.34} & \textbf{61.51} & \textbf{66.42} & \textbf{71.35} & 54.60 & \textbf{73.15}\\
\bottomrule
    \end{tabular}}
    \caption{MMDG analysis on EPIC-Kitchens and HAC using video, flow data. 'Base' denotes vanilla multi-modal joint training without domain generalization. Parentheses indicate training modalities: V (Video) and F (Flow). 'Video', 'Flow' and 'Video-Flow' represent uni-modal and multi-modal testing. Results are averaged by using each domain as target.
}
    \label{tab:sup_va_compete}
\end{table*}

% \begin{table}[h]
% \centering
% \resizebox{0.6\linewidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{4}{c}{\textbf{EPIC-Kitchens}} 
% \cmidrule(lr){2-5} \\
% \textbf{Method} & Video & Audio & Flow & V-A-F\\
% \midrule
% Base(V) &  58.73 & - & - & -\\
% Base(A) &  - & 40.04 & - & -\\
% Base(F) &  - & - & 52.61 & -\\
% Mixup(V) & 56.30 & - & - & -\\
% Mixup(A) &  - &  40.35 & - & -\\
% Mixup(F) &  - & - &  58.85 & -\\
% JiGen(V) &  58.73 & - & - & -\\
% JiGen(A) &  - & 40.04 & - & -\\
% JiGen(F) &  - & - & 52.61 & -\\
% \midrule
% Base(VAF) &  - & - & - & 61.20\\
% Mixup(VAF) &  - & - & - & 61.20\\
% JiGen(VAF) &  - & - & - & 61.20\\
% \bottomrule
% \end{tabular}
% }
% \caption{Modal_compete}
% \label{tab:epic-dg2}
% \end{table}
